Part Segmentation and Motion Estimation for Articulated Objects with Dynamic 3D Gaussians

Part segmentation and motion estimation are two fundamental problems for articulated object motion analysis. In this paper, we present a method to solve these two problems jointly from a sequence of observed point clouds of a single articulated object. The main challenge in our problem setting is that the point clouds are not assumed to be generated by a fixed set of moving points. Instead, each point cloud in the sequence could be an arbitrary sampling of the object surface at that particular time step. Such scenarios occur when the object undergoes major occlusions, or if the dataset is collected using measurements from multiple sensors asynchronously. In these scenarios, methods that rely on tracking point correspondences are not appropriate. We present an alternative approach based on a compact but effective representation where we represent the object as a collection of simple building blocks modeled as 3D Gaussians. We parameterize the Gaussians with time-dependent rotations, translations, and scales that are shared across all time steps. With our representation, part segmentation can be achieved by building correspondences between the observed points and the Gaussians. Moreover, the transformation of each point across time can be obtained by following the poses of the assigned Gaussian (even when the point is not observed). Experiments show that our method outperforms existing methods that solely rely on finding point correspondences. Additionally, we extend existing datasets to emulate real-world scenarios by considering viewpoint occlusions. We further demonstrate that our method is more robust to missing points as compared to existing approaches on these challenging datasets, even when some parts are completely occluded in some time-steps. Notably, our part segmentation performance outperforms the state-of-the-art method by 13% on point clouds with occlusions.

==> sections/intro.tex <==
\section{Introduction}



Given a dynamic point cloud sequence of an articulated object, identifying rigid parts and their motion are the core techniques for building digital twins~\cite{jiang2022ditto}, object re-posing~\cite{noguchi2022watch}, and performing system identification in robotics. 
%While many existing methods take images or videos as inputs, leveraging their rich spatial and temporal information, point clouds pose an unique challenge due to their sparsity and lack of temporal correlation.
Many existing methods take images or videos as inputs, since visual features provide important cues for spatial and temporal relationship between different time steps. Point clouds, however, do not carry much information about temporal correlation.  
Our work is one of the few methods that simultaneously estimate a) part assignment, b) kinematic tree, and c) joint poses directly from raw 4D point cloud. % without point correspondences or any assumption on the number of parts and the underlying kinematic tree structure.
Moreover, the estimated parameters can be used to re-articulate the object to a new pose that is not seen before. 

Building re-articulable models from a sequence of observation is a challenging problem. Many existing methods simplify this problem by focusing on a single category~\cite{SMPL:2015,MANO:SIGGRAPHASIA:2017} or instances that share similar kinematic structure~\cite{wu2022casa, yao2022lassie, NEURIPS2023_a99f50fb, wu2023magicpony}. Another line of research addresses this problem by targeting objects with a known number of moving parts~\cite{jiang2022ditto,liu2023paris}. However, such assumptions limit the generalizability of these approaches to in-the-wild objects. In this paper, we remove these constraints by making no assumptions about the number of parts or the underlying kinematic tree structure, making our method more suitable for real-world applications. 


There are few recent works that tackle similar problems in a category-agnostic manner. Some methods focus on part segmentation and motion estimation, but do not build articulable models~\cite{huang2021multibodysync,yi2018deep,hayden2020nonparametric}. Some other methods rely on visual features from images or videos~\cite{Kuai_2023_CVPR,noguchi2022watch}. 
The only work that shares the same problem formulation as ours is Reart~\cite{liu2023building}. Reart proposes a two-step optimization approach by first estimating the point-part assignment and a set of unconstrained part motion. Then they extract the kinematic structure and fine tune the part motion with the estimated constraint. However, their part segmentation is only optimized at a single time step, and does not generalize to other time steps, limiting their ability to segment the same object with different poses. Moreover, existing methods that work with point clouds aim to find correspondence between points at different time steps~\cite{huang2021multibodysync, liu2023building}. However, such correspondence might not exist as the observed point clouds are independently sampled from the object at every time step. 

To address the aforementioned issues, we propose to represent the rigid parts and their motion with 3D Gaussians. Instead of solving part assignment and pose estimation with point correspondence, we build correspondence between 3D points and the Gaussians that model the point distribution of each rigid part over time. 
A key aspect of our method is the Gaussian parametrization technique inspired by the success of Gaussian Splatting~\cite{kerbl3Dgaussians}. We decouple the Gaussian parameters into rotation, translation, and scale, which allow us to effectively perform part segmentation, part motion estimation, and point transformation with minimal parameters. 
%With the optimized Gaussian parameters, part segmentation can be achieved across all observed time steps, and points can be transformed to new poses according to the Gaussian poses.

We show in the experiment section that our method outperforms existing works on two established benchmarks. Moreover, while existing approaches focus on point clouds that fully cover the object surface, less attention has been given to modeling point cloud sequence with occlusions. To fill in this gap, we extend the dataset to mimic real-world scenario by involving point occlusion. Experimental results show that our method is more robust to missing points in the observed point clouds compared to previous works. Our contributions can be summarized as follows.



\begin{compactitem} 
\item  To build a re-articulable model from raw 4D point cloud of an arbitrary articulated object, we propose a compact but effective representation to model rigid part segmentation and motion with 3D Gaussians. 
\item Compared to most existing point cloud-based methods that solely rely on point correspondence, our method that considers point distribution outperforms existing methods on established benchmarks. % by...
\item We take the first step in this research direction to building re-articulable models from point clouds with partial observations. Moreover, experiments show that our method is more robust to missing points than existing works. 
\end{compactitem}

==> sections/intro_v2.tex <==
\section{Introduction}

Given a dynamic point cloud sequence of an articulated object, identifying rigid parts and their motion are the core techniques for building digital twins~\cite{jiang2022ditto}, object re-posing~\cite{noguchi2022watch}, and performing system identification in robotics. 
\vtxt{too big of a jump -- need a transition here}
Our work simultaneously estimates a) part assignment, b) kinematic tree, and c) joint poses directly from a raw point cloud sequence of a single articulated object. 
Moreover, the estimated parameters can be used to re-articulate the object to a new pose that is not seen before. 
Unlike many existing methods, we do not make any assumption on the number of parts~\cite{jiang2022ditto,liu2023paris}, or the underlying
kinematic tree structuree~\cite{wu2022casa, yao2022lassie, NEURIPS2023_a99f50fb, wu2023magicpony}. Therefore, making our method more generalizable to in-the-wild objects and more suitable for real-world applications. 

\vtxt{this paragragph could be the transition above. So I would just move this up and talk about our work afterwards}
Building a re-articulable model from a sequence of point clouds is a challenging problem. Point clouds, unlike images or videos, do not carry much information about temporal correlation. \vtxt{reword this next sentence when you reorder the paragraphs. I would not mention our problem setup yet but justify the setup independently}Moreover, in our problem setup, the input point cloud sequence is not generated by a fixed set of moving points. Instead, each point cloud in the sequence is arbitrarily sampled from the object surface at that time step. Therefore, corresponding points might not exist across the observed point cloud sequence. This setup is realistic, as it often occurs when the object is captured from multiple sensors asynchronously, or when there are occlusions caused by different sensor viewpoints. Hence, existing methods that rely on finding point correspondences may not work well in these scenarios. 


\vtxt{you can see that in the current organization, the flow is not smooth: problem - our slolution -- problem again -- now our solution again. The restructure i describe above will solve this issue}
In this paper, instead of relying solely on point correspondences, we propose an alternative approach. Our method is based on a compact but effective representation where we represent the object as a collection of simple building blocks modeled as 3D Gaussians. These Gaussians are dynamic, where each Gaussian motion represents the motion of a single rigid part.
With our representation, part segmentation can be achieved by building correspondences between the observed points and the Gaussians. 
A key component of our method is the Gaussian parametrization technique inspired by the success of Gaussian Splatting~\cite{kerbl3Dgaussians}. We decouple the Gaussian parameters into time-dependent rotations, translations, and scales
that are shared across all time steps. This allows us to effectively perform part segmentation, part motion estimation, and point transformation with minimal parameters. 
%we propose to represent the rigid parts and their motion with 3D Gaussians. Instead of solving part assignment and pose estimation with point correspondence, we build correspondence between 3D points and the Gaussians that model the point distribution of each rigid part over time. 
%With the optimized Gaussian parameters, part segmentation can be achieved across all observed time steps, and points can be transformed to new poses according to the Gaussian poses.

We show in the experiment section \vtxt{give the section number} that our method outperforms existing works on two established benchmarks. Moreover, while existing approaches focus on point clouds that fully cover the object surface, less attention has been given to modeling point cloud sequences with occlusions. To fill in this gap, we extend the dataset to mimic real-world scenario by involving point occlusions. Experiment results show that our method is more robust to missing points in the observed point clouds compared to existing works. Our contributions can be summarized as follows. \vtxt{i would highlight this occlusion business even more and mention it in the problem setting above. Right now it reads like an after thought}



\begin{compactitem} 
\item  To build a re-articulable model from raw 4D point cloud of an arbitrary articulated object, we propose a compact but effective representation by modeling rigid part segmentation and motion with 3D Gaussians. 
\item Compared to most existing point cloud-based methods that solely rely on point correspondence, our method that considers point distribution outperforms existing methods on established benchmarks. % by...
\item We take the first step in this research direction to building re-articulable models from point clouds with partial observations. Moreover, experiments show that our method is more robust to missing points than existing works. 
\end{compactitem}


% Many existing methods simplify this problem by focusing on a single category~\cite{SMPL:2015,MANO:SIGGRAPHASIA:2017} or instances that share similar kinematic structure~\cite{wu2022casa, yao2022lassie, NEURIPS2023_a99f50fb, wu2023magicpony}. Another line of research addresses this problem by targeting objects with a known number of moving parts~\cite{jiang2022ditto,liu2023paris}. However, such assumptions limit the generalizability of these approaches to in-the-wild objects. In this paper, we remove these constraints by making no assumptions about the number of parts or the underlying kinematic tree structure, making our method more suitable for real-world applications. 


% There are few recent works that tackle similar problems in a category-agnostic manner. Some methods focus on part segmentation and motion estimation, but do not build articulable models~\cite{huang2021multibodysync,yi2018deep,hayden2020nonparametric}. Some other methods rely on visual features from images or videos~\cite{Kuai_2023_CVPR,noguchi2022watch}. 
% The only work that shares the same problem formulation as ours is Reart~\cite{liu2023building}. Reart proposes a two-step optimization approach by first estimating the point-part assignment and a set of unconstrained part motion. Then they extract the kinematic structure and fine tune the part motion with the estimated constraint. However, their part segmentation is only optimized at a single time step, and does not generalize to other time steps, limiting their ability to segment the same object with different poses. Moreover, existing methods that work with point clouds aim to find correspondence between points at different time steps~\cite{huang2021multibodysync, liu2023building}. However, such correspondence might not exist as the observed point clouds are independently sampled from the object at every time step. 



==> sections/limitation.tex <==
\section{Limitations}
Like most clustering algorithms, 
As presented, our method requires the number of clusters $m$ to be given as input. We found that the choice of $m$ matters:  
On one hand, if $m$ is significantly smaller than the actual number of parts, our method fails by trying to use a single large Gaussian to approximate the motion of multiple different parts. 
On the other hand, if it is too large, our method will over-segment a single rigid part into multiple smaller parts. In this case, we presented a method to merge neighboring parts whose relative motion falls below a predefined threshold. However, this merging process is highly sensitive to the chosen threshold and can be affected by noisy pose estimations. For instance, in the case of a cylindrical part, pose variations along the main axis may not affect part segmentation and motion estimation. However, the relative motion to other parts can be numerically large, leading to wrong merging result. 
As a more general solution, we proposed a decision criterion for choosing the best $m$ from multiple initializations. However, this solution comes with added computation time.  A better solution, which we plan to explore in the future, could be to train a network for estimating the number of clusters. 

Finally, our method implicitly assumes that the kinematic structure is acyclic. While this assumption holds for for most objects, the kinematic tree estimation module needs to be generalized when this assumption fails. 

% the presented kinematic tree estimation module does not work on objects with non-tree structures, such as tripod manipulators. In future work, we plan to incorporate information from images or surface normals to handle cyclical structures.

